SLICES, a scientific instrument for the networking community

A science is defined by a set of encyclopedic knowledge related to facts or phenomena following rules or evidenced by experimentally-driven observations. Computer Science and in particular computer networks is a relatively new scientific domain maturing over years and adopting the best practices inherited from more fundamental disciplines. The design of past, present and future networking components and architectures have been assisted, among other methods, by experimentally-driven research and in particular by the deployment of test platforms, usually named as testbeds. However, often experimentally-driven networking research used scattered methodologies, based on ad-hoc, small-sized testbeds, producing hardly repeatable results. We believe that computer networks needs to adopt a more structured methodology, supported by appropriate instruments, to produce credible experimental results supporting radical and incremental innovations. This paper reports lessons learned from the design and operation of test platforms for the scientific community dealing with digital infrastructures. We introduce the SLICES initiative as the outcome of several years of evolution of the concept of a networking test platform transformed into a scientific instrument. We address the challenges, requirements and opportunities that our community is facing to manage the full research-life cycle necessary to support a scientific methodology.

==> figures/tex/AtomD.tex <==
\begin{tikzpicture}

	\node[] at (0,0){\includegraphics[width=.40\textwidth]{figures/png/AtomD_main}};
	\node[] at (4,0) {\includegraphics[width=.40\textwidth]{figures/png/AtomD_experiments}};

\end{tikzpicture}

==> figures/tex/connectivity_life_cycle.tex <==
\begin{tikzpicture}[>=latex]

\tikzmath{\recW = 17.5; \recH = 2.4;}

\draw[-](0,\recH) -- (\recW,\recH) -- (\recW,\recH*-1) -- (0,\recH*-1) -- (0, \recH);
\draw[-](0, 0) -- (\recW, 0);

\draw[-](0.7,0) -- (0.7,\recH) node[midway, above, sloped]{Advertiser};
\draw[-](0.7,\recH*-1) -- (0.7,0) node[midway, above, sloped]{Discoverer};

\node[
	circle, 
	draw,
	minimum width=0.5cm,
	fill=black
]
(advertiser_init) at (1.5,1){};

\node[
	rectangle,
	draw,
	align=center
]
(advertiser_func) at (3.8, 1){Advertising};

\node[
	rectangle,
	draw,
	align=center
]
(advertiser_request) at (7.5, 1){Receive Connection \\ Request};

\node[
	diamond,
	draw,
	align=center
]
(advertiser_request_accept) at (11.2, 1){Accept};

\node[
	rectangle,
	draw,
	align=center
]
(advertiser_connection) at (14, 1){Establish \\ Connection};

\node[
	circle, 
	draw,
	minimum width=0.5cm,
	fill = black
]
(advertiser_end) at (16.5,1){};

\node[
	circle, 
	draw,
	minimum width=0.6cm
]
(advertiser_end_ext) at (16.5,1){};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55



\node[
	circle, 
	draw,
	minimum width=0.5cm,
	fill=black
]
(discovery_init) at (1.5,-1){};

\node[
	rectangle,
	draw,
	align=center
]
(discovery_func) at (3.8, -1){Discovering};

\node[
	diamond,
	draw,
	align=center
]
(discovery_find) at (7.5, -1){Found};

\node[
	rectangle,
	draw,
	align=center
]
(discovery_request) at (11, -1){Send \\ Resquest};

\node[
	diamond,
	draw,
	align=center
]
(discovery_request_accept) at (14, -1){Accept};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](advertiser_init) -- (advertiser_func);
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](advertiser_request) -- (advertiser_request_accept);
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](advertiser_request_accept) -- (discovery_request_accept)node[midway, above]{Yes};
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](advertiser_connection) -- (advertiser_end);
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](advertiser_request_accept.north west) to [in=15,out=165]node[above]{No} (advertiser_func.north east);

\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](discovery_init) -- (discovery_func);
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](discovery_func.north east) to [out=30,in=155] (discovery_find.north west);
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](discovery_find) -- (discovery_func)node[midway, above]{No};
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](discovery_find) -- (discovery_request)node[midway, above]{Yes};
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](discovery_request.north) to [in=-80,out=140](advertiser_request.south);
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](discovery_request_accept) -- (advertiser_connection)node[midway, right]{Yes};
\draw[->,thick, -{Stealth[length=3mm, width=2mm]}](discovery_request_accept.south west) to [in=-15,out=-170]node[midway, above]{No} (discovery_func.south east);



\end{tikzpicture}

==> figures/tex/connectivity_problem_statement.tex <==
\begin{adjustbox}{width=0.48\textwidth}% there is also 'max width' to only scale it down if it is larger
\begin{tikzpicture}

\node[
	circle,
	draw,
	dashed,
	minimum width = 6cm
]
(radio_area) at (0,0)
{};

\node[
]
(radio_area_text) at (-1,2)
{$C_{D_a}$};

\node[
	circle,
  	draw, 
  	minimum width = 1cm,
] 
(advertiser) at (0,0)
{$D_a$};

\node[
] 
(advertiser_start_direction) at (-0.5,0.7)
{};

\node[
] 
(advertiser_end_direction) at (0.5,0.7)
{};



\node[
	circle,
	draw,
	minimum width = 1cm,
	fill=white
]
(discover) at (4.7, 0)
{$D_d$};



\node[
]
(discover_start_direction) at (5.2, 0.7)
{};

\node[
]
(discover_end_direction) at (4.2, 0.7)
{};


\node[circle,draw,fill=black, minimum width = 1pt](listening) at (3, 0) {};

\node[circle,draw,fill=black, minimum width = 1pt](discovery) at (1.5, 0) {};

\node[circle,draw,fill=black, minimum width = 1pt](connecting) at (-1.5, 0) {};

\node[circle,draw,fill=black, minimum width = 1pt](transmitting) at (-3, 0) {};


\draw[->](advertiser_start_direction) -- (advertiser_end_direction) node[midway, above] {$V_{D_a}$};
\draw[->](discover_start_direction) -- (discover_end_direction) node[midway, above] {$V_{D_d}$};


\draw [|-|](3, -0.7) -- (1.5, -0.7) node[midway, below] {$T_d$};
\draw[|-|](1.5, -0.7) -- (-1.5, -0.7) node[midway, below] {$T_c$};
\draw[|-|](-1.5, -0.7) -- (-3, -0.7) node[midway, below] {$T_{up}$};
\draw[|-|](-3, -1.5) -- (3, -1.5) node[midway, below] {$T_{it}$};

\coordinate[left = 0.5cm of listening] (listening_arrow);
\draw[->](listening)--(listening_arrow);
\coordinate[left = 0.5cm of discovery] (discovery_arrow);
\draw[->](discovery)--(discovery_arrow);
\coordinate[left = 0.5cm of connecting] (connecting_arrow);
\draw[->](connecting)--(connecting_arrow);
\coordinate[left = 0.5cm of transmitting] (transmitting_arrow);
\draw[->](transmitting)--(transmitting_arrow);

\end{tikzpicture}
\end{adjustbox}


==> figures/tex/connectivity_status_timing.tex <==
\begin{tikzpicture}[>=latex]
\tikzmath{\Vpos = -0.6; \Hpos = -1;}

\node[]
(discovery_timing_init) at (0,0){Node A};

\node[]
(discovery_timing_end) at (0,-5){};


\node[]
(advertiser_timing_init) at (4 + \Hpos,0){Node B};

\node[]
(advertiser_timing_end) at (4+ \Hpos,-5){};


\node[]
(beacon_1) at (4+ \Hpos,-0.5){};

\node[]
(beacon_1_end) at (0,-1+\Vpos){};

\node[]
(beacon_2) at (4+ \Hpos,-1){};

\node[]
(beacon_2_end) at (0,-1.5+\Vpos){};

\node[]
(beacon_3) at (4+ \Hpos,-1.5){};

\node[]
(beacon_3_end) at (0,-2+\Vpos){};

\node[]
(beacon_4) at (4+ \Hpos,-2){};

\node[]
(beacon_4_end) at (0,-2.5+\Vpos){};


\node[]
(request) at (0,-1.7){};

\node[]
(request_end) at (4+ \Hpos,-2.2+\Vpos){};

\node[]
(request_2) at (4+ \Hpos,-2.4+\Vpos){};

\node[]
(request_2_end) at (0,-2.9+\Vpos*2){};

\draw [decorate, decoration = {brace, mirror, raise=4pt}] (discovery_timing_init) --  (request)node[midway, xshift=-1.3cm]{Discovering};

\draw [decorate, decoration = {brace, raise=4pt}] (advertiser_timing_init) --  (request_end)node[midway, xshift=1.3cm]{Advertising};

\draw [decorate, decoration = {brace, mirror, raise=4pt}] (request) --  (request_2_end) node[text width=1cm, midway, xshift=-1.5cm]{Requesting \\ connection};


\draw[|-|,thick](discovery_timing_init) -- (discovery_timing_end);
\draw[|-|,thick](advertiser_timing_init) -- (advertiser_timing_end);

\draw[->,thick, dashed](beacon_1) -- (beacon_1_end);
\draw[->,thick, dashed](beacon_2) -- (beacon_2_end);
\draw[->,thick, dashed](beacon_3) -- (beacon_3_end);
\draw[->,thick, dashed](beacon_4) -- (beacon_4_end);

\draw[->,thick](request) -- (request_end);
\draw[->,thick](request_2) -- (request_2_end);

\draw[->, thick,dashed](4.5+\Hpos, -2.9+\Vpos*2) -- (5.5+\Hpos, -2.9+\Vpos*2) node[pos=1.8]{Beacons};
\draw[->, thick](4.5+\Hpos, -3.5+\Vpos*2) -- (5.5+\Hpos, -3.5+\Vpos*2) node[pos=1.8]{Request};

\draw[-, thick](0.8+\Hpos, -3+\Vpos*2) -- (4+\Hpos, -3+\Vpos*2) node[pos=-0.3]{Connected};

\end{tikzpicture}

==> figures/tex/d2d_useCase.tex <==
\begin{tikzpicture}[object/.style={thin,double,<->}]
  

  \node[
  	ellipse,
  	draw, 
  	minimum width = 4.5cm, 
    minimum height = 2cm, 
    inner sep=0pt
    ] (antenna) at (0,0)
  {\includegraphics[scale=.1]{figures/icons/antenna.jpg}};
  
  \node[](ref_case_broadcasting) at (1,0){\footnotesize [2]};
  
  \node[
    inner sep=0pt
    ] (phone_1) at (1.4,0)
  {\includegraphics[scale=0.04]{figures/icons/iphone}};
  
  \node[
    inner sep=0pt
    ] (phone_2) at (3,0.7)
  {\includegraphics[scale=0.04]{figures/icons/iphone}};

  \node[](ref_case_broadcasting) at (-1,-0.3){\footnotesize [1]};
  
  \node[
    inner sep=0pt
    ] (phone_3) at (-1.4,-0.3)
  {\includegraphics[scale=0.04]{figures/icons/iphone}};
  
  \node[
    inner sep=0pt
    ] (phone_4) at (-1.5,-1.8)
  {\includegraphics[scale=0.04]{figures/icons/iphone}};
  
  \node[
    inner sep=0pt
    ] (phone_5) at (-2.5,-1.3)
  {\includegraphics[scale=0.04]{figures/icons/iphone}};
  
  \node[](ref_case_broadcasting) at (0.6,-2){\footnotesize [3]};  
  
  \node[
    inner sep=0pt
    ] (phone_6) at (1,-2)
  {\includegraphics[scale=0.04]{figures/icons/iphone}};
  
    \node[
    inner sep=0pt
    ] (multimedia) at (2,-2)
  {\includegraphics[scale=0.04]{figures/icons/multimedia}};
  
  
  \node[
    inner sep=0pt
    ] (phone_7) at (3,-2)
  {\includegraphics[scale=0.04]{figures/icons/iphone}};
  
  \draw[->,thick] (phone_2) -- (phone_1);  
  \draw[->,thick] (phone_3.south) -- (phone_4.north);
  \draw[->,thick] (phone_3.south) -- (phone_5.north east);
  
  \draw[->,thick] (phone_6.north east) to [out=30,in=150] (phone_7.north west);
  \draw[->,thick] (phone_7.south west) to [out=-150,in=-30] (phone_6.south east);
  
  
\end{tikzpicture}

==> sections/EOSC.tex <==
%#############################################################################################	
\section{Introduction to EOSC}
\label{section:EOSC}
%#############################################################################################

% 1.5.1.	Integration with EOSC infrastructure and services and international testbeds


Since SLICES aims to provide a pan-European experimental research platform by jointly utilizing the geographically dispersed computing, storage and networking RIs, it is highly important that the different RIs interacting in the experimental workflow are interoperable with each other. Similarly, existing research needs to be accessible and directly pluggable to SLICES services and sites. For example, considering a MEC use case, compute, storage and networking resources from different RIs would be used. In such a scenario, it is necessary that resource description, availability, execution and data exchange are smooth. This can only be assured if a common interoperability framework is adopted across the SLICES ecosystem so that different subsystems have a common understanding of resources, data/metadata and are on the same page with respect to the licensing, copyright and privacy requirements.  The SLICES infrastructure will be designed to ensure compatibility and integration with EOSC and existing ESFRI infrastructures, and be ready to offer advanced ICT infrastructure services to other RIs and projects, with the special focus on the FAIR data management and exchange. 

EOSC~\cite{eosc} has established itself as an important pillar in the implementation of Open science concept by accelerating the adoption of the FAIR data practices among researchers in the European Union. Integration of SLICES into European Research Infrastructure via EOSC will facilitate data sharing and reuse among SLICES partners and the larger European researchers’ community. This naturally aligns SLICES to the concepts of Open science. Interoperability-focused integration of SLICES with EOSC will make it easier for SLICES users to reap the benefits of many services and tools pertaining to diverse scientific domains that are being developed around the EOSC ecosystem. 

Therefore, it is of utmost importance to design the integration framework of SLICES with EOSC in such a way that the data exchange between SLICES and EOSC is interoperable for scientific workflow management for data storage, processing and reuse. To this end, the recommendations of the EOSC interoperability framework  are considered in great detail for the design of the  SLICES interoperability framework.

Interoperability is an essential feature of EOSC ecosystem as a federation of services and data exchange is unthinkable without interoperability among different EOSC constituents. The meaningful exchange and consumption of digital objects is necessary to generate value from EOSC, which can only be realized if different components of the EOSC ecosystem (software/machines and humans) have a common understanding of how to interpret and exchange them, what are the legal restrictions, and what processes are involved in distribution, consumption and production of them. To facilitate this, EOSC interoperability framework (EOSC-IF)~\cite{eosc-if} is defined as a generic framework for all the entities involved in the development and deployment of EOSC.

To achieve this, a dedicated interface, coined SLICES-Interoperability Framework (SLICES-IF) shall be developed. The interface will be built upon the foundations led by the European Interoperability Reference Architecture (EIRA)~\cite{eira}, where interoperability is classified at four layers, namely: (i) technical, (ii) semantic, (iii) organizational; and (iv) legal. Although the target audience for EIRA (governance and administration) was very different from the SLICES stakeholders, core principles and objectives are similar. Additionally, the different components (in particular technical and semantic) of SLICES-IF would be chosen in a such way that SLICES is fully interoperable with EOSC for uninterrupted data exchange pertaining to use of EOSC services and research data by SLICES as well as to enable the publications of SLICES infrastructure, services and data through EOSC portal. More details about the SLICES-IF interface to EOSC and external RIs is provided in SLICES-Design Study Deliverable D4.2~\cite{slices-ds-d4.2}.

%Figure: SLICES interconnection with European e-Infrastructures and digital infrastructures
\begin{figure*}[t]
    \centering
    \includegraphics{././figures/png/SLICES_interface_to_EOSC.png}
	\caption{SLICES interface to EOSC}
	\label{fig:SLICES-interface-to-EOSC}
\end{figure*}

